Understanding metric-related pitfalls in image analysis validation

Validation metrics are key for the reliable tracking of scientific progress and for bridging the current chasm between artificial intelligence (AI) research and its translation into practice. However, increasing evidence shows that particularly in image analysis, metrics are often chosen inadequately in relation to the underlying research problem. This could be attributed to a lack of accessibility of metric-related knowledge: While taking into account the individual strengths, weaknesses, and limitations of validation metrics is a critical prerequisite to making educated choices, the relevant knowledge is currently scattered and poorly accessible to individual researchers. Based on a multi-stage Delphi process conducted by a multidisciplinary expert consortium as well as extensive community feedback, the present work provides the first reliable and comprehensive common point of access to information on pitfalls related to validation metrics in image analysis. Focusing on biomedical image analysis but with the potential of transfer to other fields, the addressed pitfalls generalize across application domains and are categorized according to a newly created, domain-agnostic taxonomy. To facilitate comprehension, illustrations and specific examples accompany each pitfall. As a structured body of information accessible to researchers of all levels of expertise, this work enhances global comprehension of a key topic in image analysis validation.

==> Author-contributions.tex <==
\section*{Author contributions}
\addcontentsline{toc}{chapter}{\protect\numberline{}Author Contributions}
A.R. initiated and led the study, was a member of the Delphi core team, wrote and reviewed the manuscript, prepared and evaluated all surveys, organized all workshops, suggested pitfalls, and designed all figures.
M.D.T. was a member of the extended Delphi core team and wrote and reviewed the manuscript.
P.F.J. initiated and led the study, was a member of the Delphi core team, led the \ac{ObD} and \ac{InS} expert group, wrote and reviewed the manuscript, prepared and evaluated all surveys, organized all workshops, suggested pitfalls, and participated in surveys.
L.M.-H. initiated and led the study, was a member of the Delphi core team, wrote and reviewed the manuscript, prepared and evaluated all surveys, organized all workshops, and suggested pitfalls.
M.B. was a member of the extended Delphi core team, was an active member of the \ac{ObD} and \ac{InS} expert group, wrote and reviewed the manuscript, and participated in surveys and workshops.
M.E. was a member of the extended Delphi core team, reviewed the document, assisted in survey preparation, and participated in surveys and workshops.
D.H.-N. was a member of the extended Delphi core team and prepared all surveys.
A.E.K. was a member of the extended Delphi core team and participated in surveys.
T.R. was a member of the extended Delphi core team, was an active member of the \ac{ObD} and \ac{InS} expert group, reviewed the document, assisted in survey preparation, tested all metric examples, suggested pitfalls, and participated in surveys and workshops.
C.H.S. was an active member of the \ac{ObD} and \ac{InS} expert group, reviewed the manuscript, suggested pitfalls, tested all metric examples, and participated in surveys and workshops.
L.A. reviewed the manuscript and participated in surveys and workshops.
M.A. was an active member of the \ac{SemS} expert group and participated in surveys and workshops.
T.A. was an active member of the \ac{ObD} and \ac{InS} expert group, suggested pitfalls, reviewed the manuscript, and participated in surveys and workshops.
S.B. co-led the \ac{SemS} expert group, reviewed the manuscript, suggested pitfalls, and participated in surveys and workshops.
A.B. was an active member of the biomedical and cross-topic expert groups, reviewed the manuscript, and participated in surveys and workshops.
F.B. led the calibration expert group, suggested pitfalls, reviewed the manuscript, and participated in surveys.
M.J.C. was an active member of the \ac{ImLC} expert group and participated in surveys and workshops.
V.C. was an active member of the \ac{ImLC} and cross-topic expert groups, reviewed the manuscript, and participated in surveys and 3workshops.
J.C. reviewed the manuscript, suggested pitfalls, and participated in surveys.
E.C. led the cross topic expert group, was a member of the extended Delphi core team, wrote and reviewed the manuscript, suggested pitfalls, and participated in surveys.
B.A.C. was an active member of the \ac{ObD} and \ac{InS} expert group, reviewed the manuscript, suggested pitfalls, and participated in surveys and workshops.
K.F. was an active member of the biomedical and cross-topic expert groups and participated in surveys and workshops.
L.F. was an active member of the calibration expert group, reviewed the manuscript, suggested pitfalls, and participated in surveys.
A.G. was an active member of the calibration expert group, reviewed the manuscript, suggested pitfalls, and participated in surveys.
B.v.G. participated in surveys and workshops.
B.G. led the cross-topic expert group and was an active member of the \ac{SemS} expert group, reviewed the manuscript, suggested pitfalls, and participated in surveys and workshops.
P.G. led the \ac{ImLC} expert group, was a member of the extended Delphi core team, wrote and reviewed the manuscript, suggested pitfalls, and participated in surveys and workshops.
D.A.H. was an active member of the biomedical and cross-topic expert groups, reviewed the manuscript suggested pitfalls, and participated in surveys and workshops.
M.M.H. was an active member of the \ac{ImLC} expert group, reviewed the manuscript, and participated in surveys and workshops.
M.H. co-led the biomedical expert group, was an active member of the cross-topic expert group, reviewed the manuscript, and participated in surveys and workshops.
F.I. led the \ac{SemS} expert group, reviewed the manuscript, and participated in surveys and workshops.
P.J. co-led the cross-topic expert group, was an active member of the \ac{ObD} and \ac{InS} expert group, reviewed the manuscript, and participated in surveys and workshops.
C.E.K. was an active member of the biomedical expert group, reviewed the manuscript, and participated in surveys and workshops.
D.K. suggested pitfalls and participated in surveys.
B.K. suggested pitfalls and participated in surveys.
J.K. led the biomedical expert group, reviewed the manuscript, and participated in surveys and workshops.
F.K. suggested pitfalls and participated in surveys.
Th.K. suggested pitfalls and participated in surveys.
A.K.-S. was a member of the extended Delphi core team and was an active member of the cross-topic group.
M.K. led the \ac{ObD} and \ac{InS} expert group, reviewed the manuscript, suggested pitfalls, and participated in surveys and workshops.
An.K. was an active member of the biomedical expert group, reviewed the manuscript, and participated in surveys and workshops.
Ta.K. participated in surveys and workshops.
B.A.L. was an active member of the \ac{SemS} expert group and participated in surveys and workshops.
G.L. was an active member of the \ac{ImLC} expert group, reviewed the manuscript, and participated in surveys and workshops.
A.M. was an active member of the biomedical and \ac{SemS} expert groups, suggested pitfalls, and participated in surveys and workshops.
K.M.-H. was an active member of the \ac{SemS} expert group, reviewed the manuscript, and participated in surveys and workshops.
A.L.M. participated in surveys and workshops.
E.M. was an active member of the \ac{ImLC} expert group, reviewed the manuscript, and participated in surveys.
B.M. participated in surveys and workshops.
K.G.M.M. was an active member of the cross-topic expert group, reviewed the manuscript, suggested pitfalls, and participated in surveys and workshops.
H.M. was an active member of the \ac{ImLC} expert group, reviewed the manuscript, and participated in surveys and workshops.
B.N. was an active member of the \ac{ObD} and \ac{InS} expert group, and participated in surveys.
F.N. was an active member of the biomedical expert group and participated in surveys and workshops.
J.P. participated in surveys and workshops.
S.M.R. reviewed the manuscript, suggested pitfalls, and participated in surveys.
Na.R. participated in surveys and workshops.
M.R. led the \ac{SemS} expert group, reviewed the manuscript, suggested pitfalls, and participated in surveys and workshops.
M.A.R. led the \ac{ImLC} expert group, reviewed the manuscript, suggested pitfalls, and participated in surveys and workshops.
Ni.R. was an active member of the \ac{SemS} expert group and participated in surveys and workshops.
R.M.S. was an active member of the \ac{ObD} and \ac{InS}, the biomedical, and the cross-topic expert groups, reviewed the manuscript, and participated in surveys and workshops.
A.A.T. co-led the \ac{SemS} expert group, suggested pitfalls, and participated in surveys and workshops.
A.T. was an active member of the calibration group, reviewed the manuscript, and participated in surveys.
S.A.T. was an active member of the \ac{ObD} and \ac{InS} expert group, reviewed the manuscript, and participated in surveys and workshops.
B.v.C. was an active member of the cross-topic expert group and participated in surveys.
G.V. was an active member of the \ac{ImLC} and cross-topic expert groups, reviewed the manuscript, and suggested pitfalls.
Z.R.Y. suggested pitfalls and participated in surveys.
Al.K., J.S.-R., C.I.S., and S.S. served on the expert Delphi panel and participated in workshops and surveys.



==> Terminology.tex <==
\begin{itemize}
    \item \textbf{Bounding box:}
    A bounding box is a (typically the smallest) rectangle drawn around and completely surrounding an object to be detected.
    \item \textbf{Challenge:}
    A challenge is an international competition, commonly hosted by individual researchers, an institute, or a professional society, that aims to comparatively assess the performance of competing algorithms on an identical data set, and thus serves to validate them. This validation is a crucial step towards the translation of an algorithm into practice.
    \item \textbf{Classification task:}
    A classification task is the task of giving categorical labels to an image or parts thereof. We distinguish classification at different scales, e.g. at image level, pixel level or object level.
    \item \textbf{Confidence:} See Predicted class scores.
    \item \textbf{Continuous class scores:} See Predicted class scores.
    \item \textbf{Evaluation:} See Validation.
    \item \textbf{\ac{FPPI}@Sensitivity} Once a cutoff value for the predicted class probabilities has been set in such a way that the target metric value is achieved (here: Sensitivity), other metric values are then obtained from the corresponding fixed confusion matrix, e.g. the \ac{FPPI} at the predefined Sensitivity level, denoted as \ac{FPPI}@Sensitivity.
    \item \textbf{Hierarchical structure of classes/data:}
   A hierarchical structure of classes/data is present when classes or data are dependent on each other or paired, e.g. when data have been derived from the same patient, or from the same center. It requires interpretation and statistical efforts different from those suitable for independent data.
    \item \textbf{Hyperparameter:}
    A hyperparameter is a parameter whose value is optimized to control the training of an algorithm. In contrast to other parameters, it is not derived through the training process itself, but rather set before the training procedure.
    \item \textbf{Inference:}
    An inference is a consequence or conclusion drawn based on a model output (see Prediction) and the context. 
    \item \textbf{Instance:}
    An instance refers to a dedicated object, structure or entity in an image, such as an individual cell, tumor or medical instrument.
    \item \textbf{Image-level classification:}
    Image-level classification is the assignment of one or multiple category labels to an entire image. Disease classification on dermoscopic images or fracture detection on X-ray images are common examples.
    \item \textbf{Instance segmentation:}
    Instance segmentation is the detection and delineation of each distinct object of a particular class in an image. Cell nuclei segmentation with a subsequent goal of cell tracking or counting is an example.
    \item \textbf{Meta-information:}
    Meta-information refers to data about an image that is not explicitly contained within the image, e.g. \ac{PHI} data about the patient in radiology images.
    \item \textbf{Metric:}
    Metrics are the measures according to which performance of algorithms is quantified and validated. Depending on the domain-specific validation goal and property of interest, we distinguish between different types of metrics, e.g. reference-based (assessment of the algorithm output in comparison to the image reference) vs. non-reference based (assessment of complementary properties such as runtime or carbon footprint). Metrics can further be subdivided into different families based on their mathematical properties.
    \item \textbf{\ac{NPV}@Sensitivity} Once a cutoff value for the predicted class probabilities has been set in such a way that the target metric value is achieved (here: Sensitivity), other metric values are then obtained from the corresponding fixed confusion matrix, e.g. the \ac{NPV} at the predefined Sensitivity level, denoted as \ac{NPV}@Sensitivity.
    \item \textbf{Object detection:}
    Object detection is the detection and localization of structures of one or multiple categories in an image. The detection and bounding box-based localization of polyps in colonoscopy sequences is an example.
    \item \textbf{(Output) Calibration:} In application scenarios that involve interpreting the raw algorithm output (specifically the  predicted class scores), output calibration can be used to obtain a reliable measure of confidence associated with the decision.
    \item \textbf{\ac{PPV}@Sensitivity} Once a cutoff value for the predicted class probabilities has been set in such a way that the target metric value is achieved (here: Sensitivity), other metric values are then obtained from the corresponding fixed confusion matrix, e.g. the \ac{PPV} at the predefined Sensitivity level, denoted as \ac{PPV}@Sensitivity.
    \item \textbf{Precision:}
    Precision is a term used differently in different scientific communities. In the medical community, for example, it commonly refers to the confidence of an output. Here, we use the term to denote the \ac{PPV}.
    \item \textbf{Predicted class scores:} Modern neural network-based approaches usually output predicted class scores (also referred to as continuous class scores, confidence scores or pseudo-probabilities) between 0 and 1 for every image/object/pixel and class, indicating the probability of the image/object/pixel belonging to a specific class.
    \item \textbf{Prediction:}
    Prediction refers to the output of an algorithm. It is not used in the temporal sense in this paper.
    \item \textbf{Problem category:}
    Biomedical image analysis problems can be subdivided problem categories according to the procedures performed. The category a problem falls into informs the appropriate choice of metrics. In this paper, we focus on four problem categories: Image-level classification, Semantic Segmentation, Object Detection, and Instance Segmentation. 
    \item \textbf{Pseudo-probabilities:} See Predicted class scores.
    \item \textbf{Reference / Reference-based metrics:} We assume that the validation process is based on the comparison of the algorithm output and a \textbf{reference} (sometimes called \textbf{gold standard}), which is assumed to be close or equal to the correct result; the (often forever unknown) \textbf{ground truth}. In terms of metrics, we distinguish between \textit{reference-based metrics}~\cite{jannin2006model}, which use the image-based reference, and \textit{non-reference-based metrics} that assess complementary properties, such as runtime, memory consumption, or carbon footprint. 
    The reference, sometimes also referred to as the gold standard, is a value assumed to be close or equal to the correct result, the (often forever unknown) ground truth.
    \item \textbf{Semantic Segmentation:}
    Semantic segmentation is the assignment of one or multiple category labels to each pixel in an image. Organ segmentation in Computed Tomography (CT) images and labeling full laparoscopic image frames with all appearing structures/organs/pathologies are common examples.
    \item \textbf{Sensitivity@\ac{FPPI}} Once a cutoff value for the predicted class probabilities has been set in such a way that the target metric value is achieved (here: \ac{FPPI}), other metric values are then obtained from the corresponding fixed confusion matrix, e.g. the Sensitivity at the predefined \ac{FPPI} level, denoted as Sensitivity@\ac{FPPI}.
    \item \textbf{Sensitivity@Specificity} Once a cutoff value for the predicted class probabilities has been set in such a way that the target metric value is achieved (here: Specificity), other metric values are then obtained from the corresponding fixed confusion matrix, e.g. the Sensitivity at the predefined Specificity level, denoted as Sensitivity@Specificity.
    \item \textbf{Sensitivity@\ac{PPV}} Once a cutoff value for the predicted class probabilities has been set in such a way that the target metric value is achieved (here: Sensitivity), other metric values are then obtained from the corresponding fixed confusion matrix, e.g. the \ac{PPV} at the predefined Sensitivity level, denoted as \ac{PPV}@Sensitivity.
    \item \textbf{Specificity@Sensitivity} Once a cutoff value for the predicted class probabilities has been set in such a way that the target metric value is achieved (here: Sensitivity), other metric values are then obtained from the corresponding fixed confusion matrix, e.g. the Specificity at the predefined Sensitivity level, denoted as Specificity@Sensitivity.
    \item \textbf{Structure instance:} A structure instance refers to a dedicated object, structure or entity in an image, such as an individual cell, tumor or medical instrument.
    \item \textbf{Training/Test case:}
    The data sets used in the process of algorithm development and validation comprise training/test cases. A case refers to the data (typically an n-dimensional image, possibly enhanced with clinical context information), which is required for an algorithm to produce one result (e.g. a segmentation or classification). A training case refers to a data set that includes reference annotations and is thus used for training an algorithm. A test case refers to a data set that is used for performance assessment
    \item \textbf{Validation:}
    Validation is the process of assessing that the validated algorithm is effectively doing what it is expected to do and what it was developed for, for example that a segmentation method is actually segmenting. Evaluation is the process of assessing that the algorithm is valuable, i.e. that it brings quantifiable added value for the clinical user in a dedicated clinical context \cite{iso2000quality}. 
\end{itemize}

==> pitfall-paper/sections/old-fundamentals.tex <==
\newpage
\label{sec:fundamentals}
The present work focuses on biomedical image analysis problems that can be interpreted as a classification task at image, object or pixel level. The vast majority of metrics for these problem categories is directly or indirectly based on epidemiological principles of \acf{TP}, \acf{FN}, \acf{FP}, \acf{TN}, i.e. the \textit{cardinalities} of the so-called confusion matrix. The \ac{TP}/\ac{FN}/\ac{FP}/\ac{TN}, from now on referred to as cardinalities. In the case of more than two classes $C$ we also refer to the entries of the $C \times C$ confusion matrix as cardinalities. For simplicity and clarity in notation, we restrict ourselves to the binary case in most examples. Cardinalities can be computed for image (segment), object or pixel level. They are typically computed by comparing the prediction of the algorithm to a reference annotation. Modern neural network-based approaches typically require a threshold to be set in order to convert the algorithm output comprising predicted class scores (also referred to as continuous class scores) to a confusion matrix. For the purpose of metric recommendation, the available metrics can be broadly classified as follows (see also \citep{cao2020mcc}): 

\begin{itemize}
    \item \textbf{Counting metrics} operate directly on the confusion matrix and express the metric value as a function of the cardinalities. In the context of segmentation, they have typically been referred to as \textbf{overlap-based} metrics~\cite{taha2015metrics}. We distinguish \textbf{multi-class counting metrics}, which are defined for an arbitrary number of classes and invariant under class order, from \textbf{per-class counting metrics}, which are computed by treating one class as foreground/positive class and all other classes as background. Popular examples for the former include \textit{\ac{MCC}}, \textit{Accuracy}, and \textit{Cohen's Kappa $\kappa$}, while examples for the latter are \textit{Sensitivity}, \textit{Specificity}, \textit{\ac{PPV}}, \textit{\ac{DSC}} and \textit{\ac{IoU}}.
    \item \textbf{Multi-threshold metrics} operate on a dynamic confusion matrix, reflecting the conflicting properties of interest, such as high \textit{Sensitivity} and high \textit{Specificity}. Popular examples include the \textit{\ac{AUROC}} and \textit{\ac{AP}}.
    \item \textbf{Distance-based metrics} have been designed for semantic and instance segmentation tasks. They operate exclusively on the \ac{TP} and rely on the explicit definition of object boundaries. Popular examples are the \textit{\ac{HD}} and the \textit{\ac{NSD}}.
\end{itemize}

Depending on the context (e.g. image-level classification \textit{vs.} semantic segmentation task) and the community (e.g. medical imaging community \textit{vs.} computer vision community), identical metrics are referred to with different terminology. For example, \textit{Sensitivity}, \textit{\ac{TPR}} and \textit{Recall} refer to the same concept. The same holds true for the \textit{\ac{DSC}} and the \textit{F$_1$ Score}. The most relevant metrics for the problem categories in the scope of this paper are introduced in the following.

Most metrics are recommended to be applied per class (except the multi-class counting metrics), meaning that a potential multi-class problem is converted to multiple binary classification problems, such that each relevant class serves as the positive class once. This results in different confusion matrices depending on which class is used as the positive class. 

% \newpage
% \begin{figure}[H]
% \begin{tcolorbox}[title= Relationships between metric families, colback=white]
%     \centering
%     \includegraphics[width=1\linewidth]{pitfall-paper/images/Fig1_zoom2_v5.pdf}
%     \caption{Most popular metric families and their relationships relevant for the problem categories addressed by this paper. The vast majority of metrics is directly or indirectly based on the cardinalities of the confusion matrix. The available metrics can be broadly classified into \textbf{counting metrics} that operate directly on the confusion matrix generated for a fixed threshold, \textbf{multi-threshold metrics} that operate on a dynamic confusion matrix (depending on threshold) and \textbf{distance-based metrics} that take into account the structure contour(s) or other spatial information, such as the structure center. Further abbreviations: \acf{AUROC}, \acf{AP}, \acf{DSC}, \acf{FPPI}, \acf{FPR}, \acf{HD}, \acf{IoU}, \acf{NSD}, \acf{PPV}, \acf{TNR}, \acf{TPR}.}
%     \label{fig:metric-families}
% \end{tcolorbox}
% \end{figure}

%\acresetall
\subsection{Image-level Classification}
\label{sec:fundamentals_ilc}

\textbf{Image-level classification} refers to the process of assigning one or multiple labels, or \textit{classes}, to an image. If there is only one class of interest (e.g. cancer \textit{vs.} no cancer), we speak of \textit{binary classification}, otherwise of \textit{categorical classification}. Modern algorithms usually output \textbf{predicted class probabilities} (or continuous class scores) between 0 and 1 for every image and class, indicating the probability of the image belonging to a specific class. By introducing a threshold (e.g. 0.5), predictions are considered as positive (e.g. cancer = true) if they are above the threshold or negative if they are below the threshold. Afterwards, predictions are assigned to the cardinalities (e.g. a cancer patient with prediction cancer = true is considered as \ac{TP}) \cite{davis2006relationship}. The most popular classification metrics are counting metrics, operating on a confusion matrix with fixed threshold on the class probabilities, and multi-threshold metrics, as detailed in the following. 

\paragraph{\textbf{Counting metrics}} As stated previously, counting metrics rely on the confusion matrix. We distinguish between per-class and multi-class counting metrics.

Popular per-class counting metrics include the Sensitivity, measuring the capability of an algorithm to classify truly positive samples, Specificity, measuring the capability of an algorithm to classify truly negative samples, ....

The \textit{Sensitivity} (also referred to as \textit{Recall}, \textit{\ac{TPR}} or \textit{Hit rate}) focuses on the actual positives (\ac{TP} and \ac{FN}) and represents the fraction of positives that were correctly detected as such. In contrast, \textit{\ac{PPV}} (or \textit{Precision}) divides the \ac{TP} by the total number of predicted positive cases, thus aiming to represent the probability of a positive prediction corresponding to an actual positive. A value of 1 would imply that all positive predicted cases are actually positives, but it might still be the case that positive cases were missed. Please note that the term \textit{Precision} has multiple meanings. In the context of computer assisted interventions, for example, it typically refers to the measured variance. Hence, the usage of its synonym \textit{\ac{PPV}} may be preferred.

In analogy to the \textit{Sensitivity} for positives, \textit{Specificity} (also referred to as \textit{Selectivity} or \textit{\ac{TNR}}) focuses on the negative cases by computing the fraction of negatives that were correctly detected as such. Similarly to the \textit{\ac{PPV}}, the \textit{\ac{NPV}} divides the \ac{TN} by the total number of predicted negative cases and measures how many of the predicted negative samples were actually negative. \textit{Specificity} and \textit{\ac{NPV}} require the definition of \ac{TN} cases, which is not always possible. In object detection tasks, for example (see Sec.~\ref{sec:fundamentals_od}), \ac{TN} are typically ill-defined and not provided. Therefore, these measures can not be computed in those cases. 

\textit{\ac{PPV}} and \textit{\ac{NPV}} provide quantities of direct interest to the medical practitioner, namely the probability of a certain event given the prediction of the classifier. However, unlike \textit{Sensitivity} and \textit{Specificity}, they are not only functions of the classifier but also of the study population. Hence, one cannot extrapolate from one population to another, e.g. from a case-control study to the general population without correcting for prevalence. In the case of the prevalence being unequal to 0.5, prevalence correction should be applied.

Reporting of a single metric such as \textit{Sensitivity}, \textit{\ac{PPV}} or \textit{Specificity} can be highly misleading because, for example, non-informative classifiers can achieve high values on imbalanced classes. The \textit{F$_1$ Score} (also known as \textit{\ac{DSC}} in the context of segmentation), overcomes this issue by representing the harmonic mean of \textit{\ac{PPV}} and \textit{Sensitivity} and therefore penalizing extreme values of either metric~\cite{hicks2021evaluation}, while being relatively robust against imbalanced data sets~\cite{Sun2009imbalanced}. The \textit{F$_1$ Score} is a specification of the \textit{F$\beta$ score}, which adds a weighting between \textit{\ac{PPV}} and \textit{Sensitivity}. For higher values of $\beta$, \textit{Sensitivity} is given a higher weight over \textit{\ac{PPV}}, which might be desired depending on the application. More specifically, the \textit{F$\beta$ Score} weights between \ac{FP} and \ac{FN} samples. Another metric which combines the metrics above is the \ac{LR+}, which is the ratio of the \textit{Sensitivity} and 1-\textit{Specificity} (\textit{\ac{FPR}}). This metric is described as the "probability that a positive test would be expected in a patient divided by the probability that a positive test would be expected in a patient without a disease" \citep{shreffler2020diagnostic}. It is defined as odds ratio and therefore invariant to the prevalence \citep{vsimundic2009measures}.

All of the metrics presented so far are bounded between 0 and 1 with 1 representing a perfect value and 0 the worst possible prediction of this metric. However, all of them rely on the definition of the positive class, which may be straightforward in some cases but can be based on a rather arbitrary choice in others. Notably, metric values may be completely different depending on the choice of positive class \cite{powers2020evaluation}.

To overcome the need for selecting one class as the positive class, other metrics have been suggested that can be based on all entries of a \textit{multi-class} confusion matrix, in which each class is assigned a row and a column of the matrix. The \textit{Accuracy} is one of the most commonly used metrics and measures the ratio between all correct predictions (\ac{TP} and \ac{TN}) and the total number of samples. \textit{Accuracy} is not robust against imbalanced data sets, and is therefore often replaced by the more robust \textit{\ac{BA}} that averages the \textit{Sensitivity} over all classes \cite{grandini2020metrics}. For two classes, the metric averages \textit{Sensitivity} and \textit{Specificity}. An alternative is \textit{Youden's Index J} or \textit{\ac{BM}}, similarly summing up \textit{Sensitivity} per class (or for two classes, summing up \textit{Sensitivity} and \textit{Specificity}). Note that \textit{Youden's Index J} and \textit{\ac{BA}} are closely related and can directly be calculated from the other as $J = 2BA - 1$ and $BA = (J+1)/2$. Both, \ac{BA} and \textit{Youden's Index J} are not dependent on the prevalence.

The \textit{\ac{MCC}}, also known as \textit{Phi Coefficient}, measures the correlation between the actual and predicted class. The metric is bounded between -1 and 1, with high positive values referring to a good prediction which can only be achieved when all cardinalities are good, i.e. with a low number of \ac{FP}/\ac{FN} and high \ac{TP}/\ac{TN}. Another popular metric is \textit{Cohen's Kappa $\kappa$}, which calculates the agreement between the reference and prediction while incorporating information on the agreement by chance. It is therefore a form of chance-corrected \textit{Accuracy}. Similarly to \textit{\ac{MCC}}, it incorporates all values of the confusion matrix and is bounded between -1 and 1. In contrast to \textit{\ac{MCC}}, negative values do not indicate anti-correlation, but less agreement than expected by chance. \textit{Cohen's Kappa $\kappa$} can be generalized by introducing a weighting scheme for the cardinalities in the \textit{Weighted Cohen's Kappa $\kappa$} metric. For those three metrics, a value of 0 refers to a prediction which is not better than random guessing. 

All of the presented binary counting metrics can be transferred to the multi-class case~\cite{hossin2015review, grandini2020metrics}, where \textit{\ac{MCC}} and \textit{(Weighted) Cohen's Kappa $\kappa$} have explicit definitions, whereas the others become the implicit result of an aggregation across a rotating one-versus-the-rest binary perspective for each of the classes.


%such as focusing on the positives (like \textit{Sensitivity} or \textit{\ac{PPV}}) or negatives (like \textit{Specificity} or \textit{\ac{NPV}}). 
\paragraph{\textbf{Multi-threshold metrics}}
The classical counting metrics presented above rely on fixed thresholds to be set on the predicted class probabilities (if available), resulting in them being based on the cardinalities of the confusion matrix.\textbf{ Multi-threshold metrics} overcome this limitation by calculating metric scores based on multiple thresholds. For instance, to emphasize how well a prediction distinguishes between the positive and negative class, the \textit{\ac{AUROC}} can be utilized. The \textit{\ac{ROC}} curve plots the \textit{\ac{FPR}}, which is equal to $1-\text{\emph{Specificity}}$, against the \textit{Sensitivity} for multiple thresholds of the predicted class probabilities, contrarily to just choosing one fixed threshold. For computation of the ROC curve, the class scores can be ordered in descending order and each score regarded as a potential threshold. For each threshold, the resulting \textit{Sensitivity} and \textit{Specificity} are computed, and the resulting tuple is added to the \textit{\ac{ROC}} curve as one point; note that the lower the threshold, the higher the \textit{Sensitivity} but the lower (potentially) the \textit{Specificity}. This leads to a monotonic increase of the curve. To interpolate between all points, i.e. to approximate the values between the calculated \textit{Sensitivity} and \textit{Specificity} tuples, a simple linear interpolation can be employed by drawing a line between each pair of points~\cite{davis2006relationship}. An optimal classifier would lead to \textit{Sensitivity} and \textit{Specificity} of 1 (1-\textit{Specificity} of 0), therefore corresponding to a single point $(0,1)$ on the \textit{\ac{ROC}} curve. In contrast, a classifier with no skill level (random guessing) would result in a diagonal line from $(0,0)$ to $(1,1)$. The area under the \textit{\ac{ROC}} curve is referred to as \textit{\ac{AUROC}}, also called \textit{AUC ROC} or simply \textit{AUC}.

\textit{\ac{AUROC}} comes with two advantages: threshold and scale invariance. \textit{\ac{AUROC}} measures the quality of the predictions regardless of the threshold, as it is calculated over a number of thresholds. Furthermore, \textit{\ac{AUROC}} does not focus on the absolute values of predictions, but rather on how well they are ranked. However, those properties are not always desired. If a specific penalization of \ac{FP} or \ac{FN} is desired, \textit{\ac{AUROC}} is not the best metric choice as it is invariant to the threshold. If the predicted class probabilities are intended to be well calibrated, the scale invariance feature will prevent from doing so.

Per definition, \textit{\ac{AUROC}} measures the complete area under the \textit{\ac{ROC}} curve. If only a specific range is of interest, a partial or ranged \textit{\ac{AUROC}} can also be computed \cite{ma2013use}. Similarly, metrics can be assessed at a certain point of the \textit{\ac{ROC}} curve, for example the \textit{Sensitivity} value at a specific score of the \textit{Specificity} (e.g. 0.9), also referred to as \textit{Sensitivity@Specificity}. This approach can similarly be used for other curve measures, e.g. the \textit{\ac{PR}} curve, introduced in Sec.~\ref{sec:fundamentals_od}. Please note that we will use the synonyms \textit{Precision} instead of \textit{\ac{PPV}} and \textit{Recall} instead of \textit{Sensitivity} in the case of the \textit{\ac{PR}} curve, given that this term is commonly used.

\newpage
\subsection{Semantic Segmentation}
\label{sec:fundamentals_ss}
\textbf{Semantic segmentation} is commonly defined as the process of partitioning an image into multiple segments/regions. To this end, one or multiple labels are assigned to every pixel such that pixels with the same label share certain characteristics. Semantic segmentation can therefore also be regarded as pixel-level classification. As in image-classification problems, predicted class probabilities are typically calculated for each pixel deciding on the class affiliation based on a threshold over the class scores \cite{asgari2021deep}. In semantic segmentation problems, the pixel-level classification is typically followed by a post-processing step, in which connected components are defined as objects, and object boundaries are created accordingly. Semantic segmentation metrics can roughly be classified into three classes: (1) counting metrics or overlap-based metrics, for measuring the overlap between the reference annotation and the prediction of the algorithm, (2) distance-based metrics, for measuring the distance between object boundaries, and (3) problem-specific metrics, measuring, for example, the volume of objects.

\paragraph{\textbf{Counting metrics}} The most frequently used segmentation metrics are \textbf{counting metrics}. In the context of segmentation they are also referred to as \textbf{overlap metrics}, as they essentially measure the overlap between a reference mask and the algorithm prediction. According to a comprehensive analysis of biomedical image analysis challenges~\cite{maier2018rankings}, the \textit{\ac{DSC}} \citep{dice1945measures} is the by far most widely used metric in the field of medical image analysis. It yields a value between 0 (no overlap) and 1 (full overlap). The \textit{\ac{DSC}} is identical to the \textit{F$_1$ Score} and closely related to the \textit{\ac{IoU}}, which is identical to the \textit{Jaccard Index}:

If the structure center or center line is of particular interest (e.g. in cells or vessels), \textbf{connectivity metrics} come into play, which measure the agreement of the center line between two objects. This is of special interest if linear or tube-like objects are present in a data set, for example in brain vascular analysis. In these cases, over- or undersegmentation are typically not of special interest, with the focus rather being on connectivity or network topology. For this purpose, the \textit{\ac{clDice}} \cite{shit2021cldice} has been designed. For computation, the reference and prediction skeletons need to be extracted from the binary masks. Multiple approaches have been proposed, as described in \cite{shit2021cldice}. The \textit{\ac{clDice}} is then defined as the harmonic mean of \textit{Topology Precision} and \textit{Topology Sensitivity}. The \textit{Topology Precision} measures the ratio of the overlap of the skeleton of the prediction skeleton and the reference mask and the skeleton of the prediction. Similarly to \textit{Precision}, it measures the \ac{FP} samples. On the other hand, \textit{Topology Sensitivity} incorporates \ac{FN} samples by measuring the ratio of the overlap of the skeleton of the reference and the prediction mask and the reference skeleton. 

\paragraph{\textbf{Distance-based metrics}} Overlap-based metrics are often complemented by \textbf{distance-based metrics} that operate exclusively on the \ac{TP} and compute one or several distances between the reference and the prediction. Apart from a few exceptions, distance-based metrics are often \textbf{boundary-based metrics} which focus on assessing the accuracy of object boundaries. According to~\cite{maier2018rankings}, the \textit{\ac{HD}} and its 95\% percentile variant (\textit{\ac{HD95}})~\citep{huttenlocher1993comparing} are the most commonly used boundary-based metrics. The \textit{\ac{HD}} calculates the maximum of all shortest distances for all points from one object boundary to the other, which is why it is also known as the \textit{Maximum Symmetric Surface Distance} \cite{yeghiazaryan2018family}. The \textit{\ac{HD95}} calculates the 95\% percentile instead of the maximum, therefore disregarding outliers. Another popular metric is the \textit{\ac{ASSD}}, measuring the average of all distances for every point from one object to the other and vice versa \citep{van20073d, yeghiazaryan2018family}. However, if one boundary is much larger than the other, it will impact the score much more. This is avoided by the \textit{\ac{MASD}} \cite{benevs2015performance}, which treats both structures equally by computing the average distance from structure $A$ to structure $B$ and the average distance from structure $B$ to structure $A$ and averaging both. For the \textit{\ac{HD}(95)}, \textit{\ac{MASD}} and \textit{\ac{ASSD}} metrics, a value of 0 refers to a perfect prediction (distance of 0 to the reference boundary), while there exists no fixed upper bound. The \textit{Boundary \ac{IoU}} is another option for measuring the boundary quality of a prediction. It measures the overlap between prediction and reference up to a certain width (which is controlled by the width parameter $d$) (see Sec.~\ref{sec:fundamentals_od} for details) and is bounded between 0 and 1.

A major problem related to boundary-based metrics are the error-prone reference annotations. In fact, domain experts often disagree on the definition and annotation of objects and their boundaries \cite{joskowicz2019inter}. While the  \textit{\ac{HD}(95)} and \textit{\ac{ASSD}} are not robust with respect to uncertain reference annotations, the \textit{\ac{NSD}} was explicitly designed for this purpose as a hybrid metric between boundary-based and counting-based approaches. Known uncertainties in the reference as well as acceptable deviations of the predicted boundary from the reference are captured by a threshold $\tau$ \cite{nikolov2021clinically}. Only boundary parts within the border regions defined by $\tau$ are counted as \ac{TP}. The metric is bounded between 0 (no boundary overlap) and 1 (full boundary overlap), so that it can be interpreted similarly to the classical \textit{\ac{DSC}} (though restricted to the boundary). Please note that $\tau$ is another important hyperparameter which should be chosen wisely, based on inter-rater agreement, for example.

\paragraph{\textbf{Problem-specific segmentation metrics}} 
While overlap-based metrics and distance-based metrics are the standard metrics used by the general computer vision community, biomedical applications often have special domain-specific requirements. In medical imaging, for example,  the actual volume of an object may be of particular interest (for example tumor volume). In this case, \textbf{volume metrics} such as the \textit{Absolute} or \textit{Relative Volume Error} and the \textit{Symmetric Relative Volume Difference} can be computed \cite{nai2021comparison}. 

\newpage
\subsection{Object Detection}
\label{sec:fundamentals_od}
\textbf{Object detection} refers to the detection of one or multiple objects (or: instances) of a particular class (e.g. lesion) in an image \cite{lin2014microsoft}. The following description assumes single-class problems, but translation to multi-class problems is straightforward, as validation for multiple classes on object level is performed individually per class. Notably, as multiple predictions and reference instances may be present in one image, the predictions need to include localization information, such that a matching between reference and predicted objects can be performed. Important design choices with respect to the validation of object detection methods include:
\begin{enumerate}
    \item \textit{How to represent an object?} Representation is typically composed of location information and a class affiliation. The former may take the form of a bounding box (i.e. a list of coordinates), a pixel mask, or the object's center point. Additionally, modern algorithms typically assign a confidence value to each object, representing the probability of a prediction corresponding to an actual object of the respective class. Note that a confusion matrix is later computed for a fixed threshold on the predicted class probabilities.\footnote{Please note that we will use the term confidence scores analogously to predicted class probabilities in the context of object detection and instance segmentation.}
    \item \textit{How to decide whether a reference instance was correctly detected?} This step is achieved by applying the \textit{localization criterion}. This may, for example, be based on comparing the object centers of the reference and prediction or computing their overlap.
    \item \textit{How to resolve assignment ambiguities?} The above step might lead to ambiguous matchings, such as two predictions being assigned to the same reference object. Several strategies exist for resolving such cases.
\end{enumerate}
\noindent
The following sections provide details on (1) applying the localization criterion, (2) applying the assignment strategy and (3) computing the actual performance metrics.
Please note that localization performance does not regard anatomical constraints. A tumor growing invasively into neighboring structures might have good metric scores, while clinically the localization/classification/impact for the patient might be disastrous.

\paragraph{\textbf{Localization criterion}}
As one image may contain multiple objects or no object at all, the \textbf{localization criterion} or \textbf{hit criterion} measures the (spatial) similarity between a prediction (represented by a bounding box, pixel mask, center point or similar) and a reference object. It defines whether the prediction \textit{hit/detected} (\ac{TP}) or \textit{missed} (\ac{FP}) the reference. Any reference object not detected by the algorithm is defined as \ac{FN}. Please note that \ac{TN} are not defined for object detection tasks, which has several implications on the applicable metrics, as detailed below. 

There are multiple ways to define the localization or hit criterion. Popular center-based localization criteria are (a) \textit{the center-cover criterion}, for which the reference object is considered hit if the center of the reference object is inside the predicted detection, (b) the \textit{distance-based hit criterion}, which considers a \ac{TP} if the distance $d$ between the center of the reference and the detected object is smaller than a certain threshold $\tau$ and (c) the \textit{center-hit criterion}, which holds true if the center of the predicted object is inside the reference bounding box or mask.

The most commonly used overlap-based hit criterion is determined by computing the \textit{\ac{IoU}} \citep{jaccard1912distribution}. The prediction is considered as \ac{TP} if the overlap is larger than a certain threshold (e.g. 0.3 or 0.5) and as \ac{FP} otherwise. If bounding boxes are considered, the \textit{\ac{IoU}} is computed between the reference and predicted bounding boxes (\textit{Box IoU}). For more fine-grained annotations in form of a pixel mask, the \textit{\ac{IoU}} may be computed for the complete mask (\textit{Mask IoU}). The \textit{Mask IoU} is less sensitive to structure boundary quality in larger objects. This is due to the fact that boundary pixels will increase linearly while pixels inside the structure will increase quadratically with an increase in structure size. The \textit{Boundary IoU} measures the \textit{\ac{IoU}} of two structures for mask pixels within a certain distance $d$ from the structure boundaries \cite{cheng2021boundary}.

The localization criterion should be carefully chosen according to the underlying motivation and research question and depending on the available coarseness of annotations. However, it should be noted that annotations of a lower resolution will result in an information loss. For example, the \textit{Box IoU} is sometimes used although pixel-mask annotations are available because algorithms are expected to output rough localization in the shape of boxes. Such a simplification might cause problems if structures are not well-approximated by a box shape, or if structures can overlap causing multi-component masks. Lastly, it should be noted that the decision for a cutoff value on the localization criterion leads to instabilities in the validation. For this reason, it is common practice in the computer vision community to average metrics over multiple cutoff values (default for \textit{\ac{IoU}} criteria: 0.50:0.05:0.95 \cite{lin2014microsoft}). Generally speaking, the cutoff values should be chosen according to the driving biomedical question. For example, if particular interest lies on the exact outlines, higher thresholds should be chosen. On the other hand, for noisy reference standards, a low cutoff value is preferable.

\paragraph{\textbf{Assignment strategy}}
The localization criterion alone is not sufficient to extract the final confusion matrix based on a fixed threshold for the predicted class probabilities (confidence scores), as ambiguities can occur. For example, two predictions may have been assigned to the same reference object in the localization step, or vice versa. These ambiguities need to be resolved in a further \textbf{assignment step}. 

This assignment and thus the resolving of potential assignment ambiguities can be done via different strategies. The most common strategy in the computer vision community is the \textit{Greedy by Score} strategy \cite{everingham2015pascal}. All predictions in an image are ranked by their predicted class probability and iteratively (starting with the highest probability) assigned to the reference object with the highest localization criterion for this prediction. The selected reference object is subsequently removed from the process since it can not be matched to any other prediction (unless double assignments are allowed). The \textit{Hungarian Matching} \cite{kuhn1955hungarian} is associated with a cost function, usually depending on the localization criterion, which is minimized to find the optimal assignment of predictions and reference. In the biomedical domain, more sophisticated matching strategies are often avoided by setting the localization criterion threshold to \textit{\ac{IoU}} > 0.5 and only allowing non-overlapping object predictions (which inherently avoids matching conflicts). In the case of a high ratio of touching reference objects and common non-split errors, meaning that one prediction overlaps with multiple reference objects, the Intersection over Reference (\textit{IoR}) \cite{matula2015cell} might be considered as an alternative to \textit{\ac{IoU}} \cite{matula2015cell}.


% For the \textbf{classification of objects}, the detection algorithm typically provides a classification by assigning a \textbf{confidence score} for every object bounding box, pixel mask, center point or similar, which again will be translated into cardinalities using a threshold (cf. Sec.~\ref{sec:fundamentals_ilc}). 
\newpage
\paragraph{\textbf{Metric computation}}
Similar to image-level classification and semantic segmentation algorithms, object detection algorithms are commonly assessed with counting metrics, assuming a fixed confusion matrix. However, one of the most popular object detection metrics is the multi-threshold metric \textit{\acf{AP}} \citep{lin2014microsoft}, which is the area under the \textit{\acf{PR}} curve for a certain interpolation scheme. The \textit{\ac{PR}} curve is computed similarly to the \textit{\ac{ROC}} curve by scanning over confidence thresholds and computing the \textit{Precision (\ac{PPV})} and \textit{Recall (Sensitivity)} for every threshold. Note in this context that the popular \textit{\ac{ROC}} curve is not applicable in object detection tasks because \ac{TN} are not available. Also, while the ROC curve is monotonically rising, this behavior may not be expected from the \textit{\ac{PR}} curve, which typically features a zigzag shape. Specifically "as the level of \textit{Recall} varies, the \textit{Precision} does not necessarily change linearly due to the fact that \ac{FP} replaces \ac{FN} in the denominator of the \textit{Precision} metric." \cite{davis2006relationship}. A linear interpolation would therefore be overly optimistic, which is why more complex interpolation is needed, as detailed in \cite{davis2006relationship}. 

The area under the \textit{\ac{PR}} curve is typically calculated as the \textit{\ac{AP}} implying a conservative simplification of curve interpolation,

\begin{equation}
    \text{\emph{AP}} = \sum_i (R_i - R_{i-1})P_i,
\end{equation}
with $R_i$ and $P_i$ denoting the \textit{Recall} and \textit{Precision} at the $i$th threshold\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.metrics.average_precision_score.html}}. For the \textit{\ac{PR}} curve, an optimal model would lead to \textit{Recall (Sensitivity)} and \textit{Precision (\ac{PPV})} of 1, therefore being the point $(1,1)$ on the \textit{\ac{PR}} curve. Conversely, a model with no skill level (random guessing) would result in a horizontal line with a precision proportional to the portion of positive samples, i.e. the prevalence. For computation of the metric (for a given class), the predictions are sorted in descending order of the confidence for each prediction (for that class). For each possible confidence threshold, the cardinalities are computed and the resulting tuple of \textit{Recall (Sensitivity)} and \textit{Precision} is added to the curve. In the case of multiple classes, the \textit{\ac{AP}} is calculated per class and averaged to get the \textit{\ac{mAP}} score.

In contrast to drawing the \textit{\ac{PR}} curve and computing the \textit{\ac{AP}}, \textit{\ac{FROC}} curve is often favoured in the clinical context due to its easier interpretability. It operates at object level and plots the average number of \textit{\ac{FPPI}} (in contrast to the \textit{\ac{FPR}}) against the \textit{Sensitivity} \cite{chakraborty2019analysis, van2010comparing}. The \textit{\ac{FROC} Score}, measured as the area under the \textit{\ac{FROC}} curve, however, is not bounded between 0 and 1 and the employed \textit{\ac{FPPI}} scores vary across studies, such that there exists no standardized definition of an area under the respective curve. Overall, the decision between the two metrics often boils down to a decision between a standardized and technical validation versus an interpretable and application-focused validation. 

%Integrate above?In contrast to \textit{\ac{AP}}, the \textit{\ac{FROC}} takes into account the total number of images in the data set. 

\newpage
\paragraph{Counting cardinalities at different scales}
In image-level classification problems, validation is naturally performed on the entire data set, while segmentation typically relies on computing metrics for each image and then aggregating metric values. This latter approach is not applicable in object detection in a straightforward manner because of the relatively small number of samples per image (typically a few objects rather than thousands of pixels). In the per-image aggregation approach, special care needs to be taken in the case of an empty reference or prediction. 

%A per image analysis of object detection problems means that aggregation of GT-matched objects (TP, FP, FN) is performed per image instead of per entire dataset implying that an evaluation score for for associated metrics (e.g. recall, precision, F1,...) is computed per image. 

%Importantly, here GT matching (the process of defining TP,FP,FN)  is performed on object-level (object-level predictions versus object-level reference) and only subsequent aggregation/counting is performed on a per-image basis. This procedure is not to be confused with “image-level” evaluation, where GT matching happens on image-level (image-level prediction versus image-level reference label). 

%In contrast to the “per entire dataset” evaluation on object-level, the per image analysis naturally introduces a weighting as to which errors (FP and FN) are penalized higher the fewe objects (i.e. predictions for FP penalties, and reference objects for FN penalties) are present in an image. This reweighting of penalties might be of interest depending on the application: For instance, a single FP in an "empty" patient should receive a higher penalty than the tenth FP in a patient with several tumors, as the latter has no relevance for the subsequent decision/diagnosis. 

%Evaluating object-level cardinalities of TP, FP, FN on a per-image basis comes with several pitfalls one should be careful about: 1) The re-weighting of penalties in a per-image counting compared to per-dataset counting introduces drastic sensitivities between single objects and output metrics (e.g. predicting just one FP in an “empty" image flips the F1-score from 1 to 0). 2) Per-image metrics like sensitivity, precision, or F1-score are sensitive to conventions on how to deal with NaNs: There are two scenarios where NaNs in counting metrics can occur: 1) Missing reference objects will lead to NaN in the calculation of recall and missing predictions will lead to NaN in the calculation of precision. The user is required to decide how to deal with such cases (see XXX for recommendations on how to deal with NaNs).

A few comments on how to compute evaluation metrics while aggregating matched objects per image: 

\begin{itemize}
    \item \textbf{Counting metrics:} Computing per-class metrics such as Sensitivity, \ac{PPV}, or F$_1$ Score works intuitively by computing a score per image and averaging scores over the data set while considering the \texttt{\ac{NaN}} conventions.
    \item \textbf{Multi-threshold metrics:} While scanning over all thresholds in the data set (analogously to per data set evaluation), for every threshold the Precision (\ac{PPV}) and Recall (Sensitivity) scores are computed per image/patient (while considering the \texttt{\ac{NaN}} conventions in and averaged over the data set. The averaged Precision and Recall score pairs per threshold form the \ac{PR} curve. The \ac{AP} can be computed for this curve analogously to the per-data set evaluation. The \ac{FROC} curve computation works analogously while replacing Precision per image with \ac{FPPI}. 
    \item \textbf{Single working point evaluation:} A single working point (e.g. \ac{PPV}@Sensitivity) can be retrieved based on the curves resulting from multi-threshold evaluation described above.
\end{itemize}

\subsection{Instance Segmentation}
\label{sec:fundamentals_is}
In contrast to semantic segmentation, \textbf{instance segmentation} problems distinguish different instances of the same class (e.g. different lesions). Similarly to object detection problems, the task is to detect individual instances of the same class, but detection performance is measured by pixel-level correspondences (as in semantic segmentation problems). Optionally, instances can be applied to one of multiple classes. Validation metrics in instance segmentation problems often combine common detection metrics with segmentation metrics applied per instance.  
 
If detection and segmentation performance should be assessed simultaneously in a single score, the \textit{\ac{PQ}} metric can be utilized \cite{kirillov2019panoptic}. The segmentation quality is assessed by averaging the \textit{\ac{IoU}} scores for all \ac{TP} instances. While this part alone would neglect \ac{FP} and \ac{FN} predictions, it is multiplied with the detection quality, which is equal to the \textit{F$_1$ score}. For perfect segmentation results, i.e. an average \textit{\ac{IoU}} of 1, the \textit{\ac{PQ}} would simply equal the \textit{F$_1$ Score}. In other words, while segmentation quality in the \textit{F$_1$ Score} is merely integrated via a hard cutoff during localization (e.g. \textit{\ac{IoU}} > 0.5) affecting the counts of \ac{TP} versus \ac{FP} and \ac{FN}, \textit{\ac{PQ}} allows for a continuous measurement of segmentation quality by 1) employing a lose prior localization criterion (e.g. \textit{\ac{IoU}} > 0, i.e. any prediction overlapping with a reference instance is treated as \ac{TP}) and 2) replacing the simple counting of \ac{TP} by adding up the continuous \textit{\ac{IoU}} scores per \ac{TP}. \textit{\ac{PQ}} was introduced for panoptic segmentation problems that are a combination of semantic and instance segmentation \cite{kirillov2019panoptic}. It is computed per class (including background classes) and can therefore be directly used for instance segmentation problems by only assessing the foreground instances. If needed, the background quality can also be assessed.

\textit{\ac{PQ}} covers segmentation and detection quality in a single score. However, this can be misleading. \textit{Prediction 1} with a perfect segmentation and poor detection achieves a \textit{\ac{PQ}} score similar to that of \textit{Prediction 2}, which detects all objects correctly (without any \ac{FP} or \ac{FN}), but only provides moderate segmentation results. If segmentation and detection quality should be assessed individually, two separate metrics - one for segmentation quality and one for detection quality - should be preferred. 

 %resulting in an instance label in addition to a class label for all non-background classes \cite{gupta2019lvis}. Thus, instance segmentation problems are a combination of object detection (detecting and localizing instances of certain classes) and semantic segmentation (pixel-wise classification rather than coarse representation). Instance segmentation problems are therefore typically validated similar to object detection tasks, with additional semantic segmentation performance metrics applied to each instance. 
 It should be noted that instance segmentation problems are often phrased as semantic segmentation problems with an additional post-processing step, such as connected component analysis \cite{rosenfeld1966sequential}. In practice, predicted class probabilities, yielded by modern segmentation algorithms, are often discarded in the post-processing step and are thus not available for subsequent validation. 

